The SDSS-V Local Volume Mapper (LVM): Data Analysis Pipeline

We introduce the Data Analysis Pipeline (DAP) for the Sloan Digital Sky Survey V (SDSS-V) Local Volume Mapper (LVM) project, referred to as the LVM-DAP. We outline our methods for recovering both stellar and emission line components from the optical integral field spectroscopy, highlighting the developments and changes implemented to address specific challenges of the data set. The observations from the LVM project are unique because they cover a wide range of physical resolutions, from approximately 0.05 pc to 100 pc, depending on the distance to the targets. This, along with the varying number of stars sampled in each aperture (ranging from zero, just one of a few, to thousands), presents challenges in using previous spectral synthesis methods and interpreting the spectral fits. We provide a detailed explanation of how we model the stellar content and separate it from the ionized gas emission lines. To assess the accuracy of our results, we compare them with both idealized and more realistic simulations, highlighting the limitations of our methods. We find that the DAP robustly correct for stellar continuum features and recover emission line parameters (e.g. flux, equivalent width, systemtic velocity and velocity dispersion) with a precision and accuracy that fulfill the requirements of the primary goal of the analysis. In addition, the recovered stellar parameters are reliable for single stars, the recovery of integrated populations is less precise. We conclude with a description of the data products we provide, instructions for downloading and using our software, and a showcase illustrating the quality of the data and the analysis on a deep exposure taken on the Huygens region at the center of the Orion Nebula.

==> table.tex <==
%----------------------------------------------------------------
\begin{table*}
\begin{center}
\caption{Emission lines considered by the LVM-DAP analysis}
\begin{tabular}{lll|lll|lll|lll|lll}\hline\hline
{\tt \#I} &$\lambda$ (\AA) & Id &
{\tt \#I} &$\lambda$ (\AA) & Id &
{\tt \#I} &$\lambda$ (\AA) & Id &
{\tt \#I} &$\lambda$ (\AA) & Id &
{\tt \#I} & $\lambda$ (\AA) & Id \\
\hline
0 &  3686.83  &   HI        & 39 &  4416.27  &   [FeII]  & 78 &  5039.10  &   [FeII]  & 117 &  6087.00  &   [FeVII]  & 156 &  8300.99  &   [NiII]  \\ 
1 &  3691.56  &   HI        & 40 &  4452.11  &   [FeII]  & 79 &  5072.40  &   [FeII]  & 118 &  6300.30  &   {\bf [OI]}  & 157 &  8308.39  &   [CrII]  \\ 
2 &  3697.15  &   HI        & 41 &  4457.95  &   [FeII]  & 80 &  5107.95  &   [FeII]  & 119 &  6312.06  &   [SIII]  & 158 &  8345.55  &   HI  \\ 
3 &  3703.85  &   HI        & 42 &  4470.29  &   [FeII]  & 81 &  5111.63  &   [FeII]  & 120 &  6363.78  &   [OI]  & 159 &  8357.51  &   [CrII]  \\ 
4 &  3711.97  &   HI        & 43 &  4471.48  &   HeI     & 82 &  5145.80  &   [FeVI]  & 121 &  6374.51  &   [FeX]  & 160 &  8359.00  &   HI  \\ 
5 &  3726.03  &   {\bf [OII]} & 44 &  4474.91  &   [FeII]  & 83 &  5158.00  &   [FeII]  & 122 &  6435.10  &   [ArV]  & 161 &  8374.48  &   HI  \\ 
6 &  3728.82  &   {\bf [OII]} & 45 &  4485.21  &   [NiII]  & 84 &  5158.90  &   [FeVII]  & 123 &  6548.05  &   {\bf [NII]}  & 162 &  8392.40  &   HI  \\ 
7 &  3734.37  &   HI        & 46 &  4562.48  &   [MgI]  & 85 &  5176.00  &   [FeVI]  & 124 &  6562.85  &   {\bf H$\alpha$}  & 163 &  8446.00  &   OI  \\ 
8 &  3750.15  &   HI        & 47 &  4571.10  &   MgI]  & 86 &  5184.80  &   [FeII]  & 125 &  6583.45  &   {\bf [NII]}  & 164 &  8467.25  &   HI  \\ 
9 &  3758.90  &   [FeVII]   & 48 &  4632.27  &   [FeII]  & 87 &  5191.82  &   [ArIII]  & 126 &  6678.15  &   HeI  & 165 &  8498.02  &   CaII  \\ 
10 &  3770.63  &   HI       & 49 &  4658.10  &   [FeIII]  & 88 &  5197.90  &   [NI]  & 127 &  6716.44  &   {\bf [SII]}  & 166 &  8502.48  &   HI  \\ 
11 &  3797.90  &   HI       & 50 &  4685.68  &   HeII  & 89 &  5200.26  &   [NI] & 128 &  6730.82  &   {\bf [SII]}  & 167 &  8542.09  &   CaII  \\ 
12 &  3819.61  &   HeI      & 51 &  4701.62  &   [FeIII]  & 90 &  5220.06  &   [FeII]  & 129 &  6855.18  &   FeI  & 168 &  8545.38  &   HI  \\ 
13 &  3835.38  &   HI       & 52 &  4711.33  &   [ArIV]  & 91 &  5261.61  &   [FeII]  & 130 &  7005.67  &   [ArV]  & 169 &  8578.70  &   [ClII]  \\ 
14 &  3868.75  &   [NeIII]  & 53 &  4713.14  &   HeI  & 92 &  5268.88  &   [FeII]  & 131 &  7065.19  &   HeI  & 170 &  8598.39  &   HI  \\ 
15 &  3888.65  &   HeI      & 54 &  4724.17  &   [NeIV]  & 93 &  5270.30  &   [FeIII]  & 132 &  7135.80  &   [ArIII]  & 171 &  8616.96  &   [FeII]  \\ 
16 &  3889.05  &   HI       & 55 &  4733.93  &   [FeIII]  & 94 &  5273.38  &   [FeII]  & 133 &  7155.14  &   [FeII]  & 172 &  8662.14  &   CaII  \\ 
17 &  3933.66  &   CaII     & 56 &  4740.20  &   [ArIV]  & 95 &  5277.80  &   [FeVI]  & 134 &  7171.98  &   [FeII]  & 173 &  8665.02  &   HI  \\ 
18 &  3964.73  &   HeI      & 57 &  4754.83  &   [FeIII]  & 96 &  5296.84  &   [FeII]  & 135 &  7236.00  &   CII  & 174 &  8727.13  &   [CI]  \\ 
19 &  3967.46  &   [NeIII]  & 58 &  4769.60  &   [FeIII]  & 97 &  5302.86  &   [FeXIV]  & 136 &  7281.35  &   HeI  & 175 &  8750.47  &   HI  \\ 
20 &  3968.47  &   CaII     & 59 &  4774.74  &   [FeII]  & 98 &  5309.18  &   [CaV]  & 137 &  7290.42  &   [FeI]  & 176 &  8862.78  &   HI  \\ 
21 &  3970.07  &   H$\epsilon$ & 60 &  4777.88  &   [FeIII]  & 99 &  5333.65  &   [FeII]  & 138 &  7291.46  &   [CaII]  & 177 &  8891.88  &   [FeII]  \\ 
22 &  4026.19  &   HeI         & 61 &  4813.90  &   [FeIII]  & 100 &  5335.20  &   [FeVI]  & 139 &  7318.92  &   [OII]  & 178 &  9014.91  &   HI  \\ 
23 &  4068.60  &   [SII]       & 62 &  4814.55  &   [FeII]  & 101 &  5376.47  &   [FeII]  & 140 &  7323.88  &   [CaII]  & 179 &  9033.45  &   [FeII]  \\ 
24 &  4076.35  &   [SII]       & 63 &  4861.36  &   {\bf H$\beta$}  & 102 &  5411.52  &   HeII  & 141 &  7329.66  &   [OII]  & 180 &  9051.92  &   [FeII]  \\ 
25 &  4101.77  &   {\bf H$\delta$} & 64 &  4881.11  &   [FeIII]  & 103 &  5412.64  &   [FeII]  & 142 &  7377.83  &   [NiII]  & 181 &  9069.00  &   {\bf [SIII]}  \\ 
26 &  4120.81  &   HeI         & 65 &  4889.63  &   [FeII]  & 104 &  5424.20  &   [FeVI]  & 143 &  7388.16  &   [FeII]  & 182 &  9123.60  &   [ClII]  \\ 
27 &  4177.21  &   [FeII]      & 66 &  4893.40  &   [FeVII]  & 105 &  5426.60  &   [FeVI]  & 144 &  7411.61  &   [NiII]  & 183 &  9226.60  &   [FeII]  \\ 
28 &  4227.20  &   [FeV]       & 67 &  4905.35  &   [FeII]  & 106 &  5484.80  &   [FeVI]  & 145 &  7452.50  &   [FeII]  & 184 &  9229.02  &   HI  \\ 
29 &  4243.98  &   [FeII]      & 68 &  4921.93  &   HeI  & 107 &  5517.71  &   [ClIII]  & 146 &  7637.52  &   [FeII]  & 185 &  9266.00  &   OI  \\ 
30 &  4267.00  &   CII         & 69 &  4924.50  &   [FeIII]  & 108 &  5527.33  &   [FeII]  & 147 &  7686.19  &   [FeII]  & 186 &  9267.54  &   [FeII]  \\ 
31 &  4287.40  &   [FeII]      & 70 &  4930.50  &   [FeIII]  & 109 &  5577.34  &   [OI]  & 148 &  7686.90  &   [FeII]  & 187 &  9399.02  &   [FeII]  \\ 
32 &  4340.49  &   {\bf H$\Upsilon$} & 71 &  4942.50  &   [FeVII]  & 110 &  5631.10  &   [FeVI]  & 149 &  7751.06  &   [ArIII]  & 188 &  9470.93  &   [FeII]  \\ 
33 &  4358.10  &   [FeII]        & 72 &  4958.91  &   {\bf [OIII]}  & 111 &  5677.00  &   [FeVI]  & 150 &  7774.00  &   OI  & 189 &  9531.10  &   {\bf [SIII]}  \\ 
34 &  4358.37  &   [FeII]        & 73 &  4972.50  &   [FeVI]  & 112 &  5720.70  &   [FeVII]  & 151 &  7891.80  &   [FeXI]  & 190 &  9545.97  &   HI  \\ 
35 &  4359.34  &   [FeII]        & 74 &  4973.39  &   [FeII]  & 113 &  5754.59  &   [NII]  & 152 &  7999.85  &   [CrII]  & 191 &  9682.13  &   [FeII]  \\ 
36 &  4363.21  &   [OIII]        & 75 &  4985.90  &   [FeIII]  & 114 &  5876.00  &   HeI  & 153 &  8125.22  &   [CrII]  &  &    &  \\ 
37 &  4413.78  &   [FeII]        & 76 &  5006.84  &   {\bf [OIII]}  & 115 &  5889.95  &   NaI  & 154 &  8229.55  &   [CrII]  & &    &  \\ 
38 &  4414.45  &   [FeII]        & 77 &  5015.68  &   HeI  & 116 &  5895.92  &   NaI  & 155 &  8236.77  &   HeII  &   &    &  \\ 
\hline
\end{tabular}\label{tab:fe_long_list}
\end{center}
List of emission lines considered in the non-parametric analysis (i.e., moment analysis), where {\tt \#I} corresponds to the index (1st column) in the tables included in the NP\_EL\_B, NP\_EL\_R and NP\_EL\_I extensions of the DAP file described in Sec. \ref{sec:DP} and Tab. \ref{tab:hdu}. The emission lines considered in the parametric analysis (i.e., those included in the {PM\_ELINES} extension of the DAP file), are indicated with a bold font. {\bf The wavelength of the emission lines have been trimmed to the 2nd decimal to fit into the table. The actual values of the wavelength should be updated electronically in the list distributed within the DAP code.}
\end{table*}
% ----------------------------------------------------------------


